Is a Caption Worth a Thousand Images? A Controlled Study for Representation Learning

The development of CLIP [Radford et al., 2021] has sparked a debate on whether language supervision can result in vision models with more transferable representations than traditional image-only methods. Our work studies this question through a carefully controlled comparison of two approaches in terms of their ability to learn representations that generalize to downstream classification tasks. We find that when the pre-training dataset meets certain criteria -- it is sufficiently large and contains descriptive captions with low variability -- image-only methods do not match CLIP's transfer performance, even when they are trained with more image data. However, contrary to what one might expect, there are practical settings in which these criteria are not met, wherein added supervision through captions is actually detrimental. Motivated by our findings, we devise simple prescriptions to enable CLIP to better leverage the language information present in existing pre-training datasets.

==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the 
  abstract and introduction accurately 
  reflect the paper's contributions and 
  scope?
  \answerYes{}
  \item Did you describe the limitations of 
  your work?
  \answerYes{See Section~\ref{sec:conclusion}.}
  \item Did you discuss any potential 
  negative societal impacts of your work?
  \answerYes{See Section~\ref{sec:conclusion}.}
  \item Have you read the ethics review 
  guidelines and ensured that your paper 
  conforms to them?
  \answerYes{}
\end{enumerate}


\item If you are including theoretical 
results...
\begin{enumerate}
  \item Did you state the full set of 
  assumptions of all theoretical results?
   \answerNA{}
        \item Did you include complete proofs 
        of all theoretical results?
        \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and 
  instructions needed to reproduce the 
  main experimental results (either in the 
  supplemental material or as a URL)? 
    \answerYes{Experimental setup details are provided in Appendix~\ref{app:setup} and code is included as part of the supplementary material.}
  \item Did you specify all the training 
  details (e.g., data splits, hyperparameters, 
  how they were chosen)?
  \answerYes{See Appendix~\ref{app:hyperparameters}.}
        \item Did you report error bars (e.g., 
        with respect to the random seed after 
        running experiments multiple times)?
        \answerYes{We report 95\% confidence intervals obtained via bootstrapping; see Appendix~\ref{app:hyperparameters}.}
        \item Did you include the total 
        amount of compute and the type of 
        resources used (e.g., type of GPUs, 
        internal cluster, or cloud provider)?
        \answerYes{See Appendix~\ref{app:compute}.}
\end{enumerate}


\item If you are using existing assets (e.g., 
code, data, models) or curating/releasing 
new assets...
\begin{enumerate}
  \item If your work uses existing assets, 
  did you cite the creators?
  \answerYes{}
  \item Did you mention the license of the 
  assets?
  \answerYes{See Appendix~\ref{app:datasets}.}
  \item Did you include any new assets 
  either in the supplemental material or as a 
  URL?
  \answerNA{}
  \item Did you discuss whether and how 
  consent was obtained from people whose 
  data you're using/curating?
  \answerNA{}
  \item Did you discuss whether the data 
  you are using/curating contains 
  personally identifiable information or 
  offensive content?
  \answerYes{See Appendix~\ref{app:datasets}.}
\end{enumerate}


\item If you used crowdsourcing or 
conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of 
  instructions given to participants and 
  screenshots, if applicable?
  \answerNA{}
  \item Did you describe any potential 
  participant risks, with links to 
  Institutional Review Board (IRB) approvals, 
  if applicable?
  \answerNA{}
  \item Did you include the estimated 
  hourly wage paid to participants and the 
  total amount spent on participant 
  compensation?
  \answerNA{}
\end{enumerate}


\end{enumerate}
